Multimodal Language Models as Text-to-Image Model Evaluators

The steady improvements of text-to-image (T2I) generative models lead to slow deprecation of automatic evaluation benchmarks that rely on static datasets, motivating researchers to seek alternative ways to evaluate T2I progress. We present Multimodal Text-to-Image Eval (MT2IE), an evaluation framework in which a single multimodal large language model (MLLM) acts as an evaluator agent, iteratively generating the evaluation prompts and scoring the resulting images. We show that MT2IE's image-text consistency scores have higher correlation with human judgment than metrics previously introduced in the literature. MT2IE generates prompts that are efficient at probing T2I model performance: closely recovering the official T2I model rankings of three structurally distinct benchmarks from just 20 generated evaluation prompts, 28-105x fewer than the benchmarks' own prompt sets. When compared to existing evaluation metrics such as CLIPScore, VIEScore, and VQAScore, MT2IE's T2I model rankings are more faithful and far more consistent across multiple evaluation seeds when using the same number of prompts. MT2IE can also adapt evaluation to the model being tested: rewriting each prompt based on the model's own measured performance to produce a bespoke per-model benchmark that still recovers the official rankings and keeps the evaluated model in an informative scoring range. We hope that these results will encourage the development of dynamic and interactive evaluation frameworks, and mitigate the deprecation of automatic evaluation benchmarks.

==> sec/3_experimental_setup.tex <==
\section{Experimental Overview}\label{sec:approach}
We demonstrate the effectiveness of using MLLMs as evaluator agents for assessing T2I image-text consistency. In \methodlong, the MLLM interacts with the T2I model by proposing text prompts and scoring the resulting generations. We show that our interactive approach enables MLLMs to effectively benchmark T2I models in two distinct settings: either by systematically generating prompts of increasing complexity or by dynamically adapting prompts based on T2I model performance.
In the following sections, we focus on evaluating image-text consistency as it directly impacts the overall visual quality of generated images \citep{pareto, imagereward, pickscore}.
Additionally, in Appendix \ref{app:aesthetic_evals} we show that \method\ is an easily generalizable framework, capable of evaluating other aspects of T2I models such as image aesthetics.
% Additionally, to demonstrate that \method\ can be easily adapted to assess other T2I properties, we also show its ability to assess image aesthetics.
We use \method\ to evaluate a total of 8 recent T2I models spanning several architectures: the latent diffusion models (LDMs) SD2.1~\citep{Rombach_2022_CVPR}, SD3~\citep{sd3}, SDXL~\citep{podell2023sdxl}, and SDXL-Turbo~\citep{sauer2025adversarial}; the flow-based model Flux~\citep{flux}; the cascaded pixel-based diffusion model DeepFloyd~\citep{deepfloyd}; Playground 2.5~\citep{playground2.5}; and PixArt-$\alpha$~\citep{pixart-alpha}.
We provide an outline of our experiments and elaborate in subsequent sections.\looseness-1


\vspace{-0.2cm}
\paragraph{Experiment 1: Validation of MLLM image-text consistency scoring capabilities.}
We validate that open-source MLLMs are capable of scoring image-text consistency on existing benchmarks without the usage of other models or fine-tuning.
Existing works that use MLLMs for end-to-end evaluation either do not use existing benchmarks or fine-tune open-source MLLMs for the task \citep{tan2024evalalign, viescore}.
Existing GQA-based benchmarks rely on a system of models for question generation and scoring; typically an LLM is used to generate questions based on a curated text prompt, the generated questions are validated by an additional LLM or question-answering model, then finally a VQA model scores the image using the generated questions \citep{dsg, vq_2, tifa, vis_prog}. % ENDED HERE
We validate that MLLMs are capable of emulating GQA-based benchmarks by generating questions about a given prompt and scoring the generated questions given the corresponding image.
We evaluate using TIFA160 \citep{tifa}, and show that a single open-source MLLM can recreate this benchmark and score questions with better correlation to human judgment.
We detail this experiment in Section~\ref{sec:contribution_1}.
% Previous VQA-based benchmarks rely on a system of models for question generation and scoring. Typically an LLM is used to generate questions based on a curated text prompt, and often the generated questions are validated by an additional LLM or question-answering model, then finally a VQA model scores the image using the generated questions \cite{dsg, vq_2, tifa, vis_prog}.
%We show that MLLMs are able to recreate, with better correlation to human judgment, existing T2I benchmarks that utilize a divide-and-conquer framework of leveraging various models for prompt decomposition and question generation, then a VQA model for image-text alignment scoring \cite{dsg, vp_eval, tifa, t2icompbench, vq_squared_(baseline)}.
% We show that a single MLLM can both recreate this existing benchmark and accurately score questions.
% The MLLMs even show better correlation with human judgements, meaning this streamlined process is both more efficient and more accurate.
% an existing T2I benchmark, TIFAv1.0 \cite{tifa}. We also employ MLLMs to emulate VQA-based benchmarks which do not rely on LLM-generated questions and instead use a single VQA model to compute the probability of answering ``yes'' to a generic prompt-related question. We demonstrate the potential of MLLMs to evaluate prompt-generation consistency in both single score and VQA-based settings and detail these experiment in


\vspace{-0.2cm}
\paragraph{Experiment 2: MLLMs to generate image-text consistency benchmarks.} After validating MLLMs' abilities to generate and score image-text consistency questions in Experiment 1, we introduce \method\, demonstrating how MLLMs can iteratively generate a full T2I benchmark and judge model image-text consistency. %explore the potential of MLLMs to operate beyond image-prompt consistency judges and validate their capabilities of generating full T2I benchmarks.
% We show that MLLMs are able to generate prompts effective for T2I model evaluation. The proposed prompts can be effectively used to score and rank state-of-the-art T2I models, removing the need for existing static datasets.
In particular, we show that from just 20 generated prompts, MLLM-generated benchmarks closely recover the official benchmark model rankings of full static benchmarks---GenEval, T2I-CompBench, and GenAIBench---far more faithfully and more consistently than baselines using an equal number of prompts.
We also show that our method is efficient, accurately ranking models with significantly fewer prompts than existing benchmarks of handwritten prompts. We detail these experiments in Section \ref{sec:mllm_genbench}.
% Additionally, we highlight the potential generalizability of \method\ by repurposing our framework to evaluate image aesthetics in Appendix \ref{app:aesthetic_evals}.


\vspace{-0.2cm}
\paragraph{Experiment 3: MLLMs to generate interactive image-text consistency benchmarks.} Beyond just generating benchmarks, we demonstrate that \method\ can act as an evaluator agent, adapting to model-specific performance. Specifically, we show that MLLMs can adjust the complexity of prompts based on model performance on previous prompts.
This enables each individual T2I model to have bespoke prompts tailored to its abilities, discussed in Section \ref{sec:adaptive}.

